Few-Shot Preference Learning for Human-in-the-Loop RL

While reinforcement learning (RL) has become a more popular approach for robotics, designing sufficiently informative reward functions for complex tasks has proven to be extremely difficult due their inability to capture human intent and policy exploitation. Preference based RL algorithms seek to overcome these challenges by directly learning reward functions from human feedback. Unfortunately, prior work either requires an unreasonable number of queries implausible for any human to answer or overly restricts the class of reward functions to guarantee the elicitation of the most informative queries, resulting in models that are insufficiently expressive for realistic robotics tasks. Contrary to most works that focus on query selection to \emph{minimize} the amount of data required for learning reward functions, we take an opposite approach: \emph{expanding} the pool of available data by viewing human-in-the-loop RL through the more flexible lens of multi-task learning. Motivated by the success of meta-learning, we pre-train preference models on prior task data and quickly adapt them for new tasks using only a handful of queries. Empirically, we reduce the amount of online feedback needed to train manipulation policies in Meta-World by 20$\times$, and demonstrate the effectiveness of our method on a real Franka Panda Robot. Moreover, this reduction in query-complexity allows us to train robot policies from actual human users. Videos of our results and code can be found at https://sites.google.com/view/few-shot-preference-rl/home.

==> preliminaries.tex <==
\section{Preliminaries} \label{sec:preliminaries}

\subsection{Preference-Based Reinforcement Learning}

% Revising this for 

As in standard RL, we consider an agent that receives state observations $s_t \in \mathcal{S}$ and takes actions $a_t \in \mathcal{A}$ with the goal of maximizing its expected cumulative discounted return $\E[\sum_t^\infty \gamma^t r_t]$ for discount factor $\gamma$.


Unlike in standard RL, in preference based RL the reward at each timestep $r_t$ is determined by a learned reward function $\hat{r}_\psi(s_t, a_t)$. As in \citet{wilson2012bayesian} we consider preferences over behavior segments $\sigma = (s_t, a_t, s_{t+1}, a_{t+1}, ..., s_{t+k-1}, s_{t+k-1})$ of $k$ states and actions. \citet{christiano2017deep} formalized a preference predictor over segments using the paired comparison model from \citet{bradley1952rank}.

\begin{equation*} \label{eq:prob}
    P[\sigma_1 \succ \sigma_2 ] = \frac{\exp \sum_t \hat{r}_\psi(s_t^{0}, a_t^{0})}{\exp \sum_t \hat{r}_\psi(s_t^{0}, a_t^{0}) + \exp \sum_t \hat{r}_\psi(s_t^{1}, a_t^{1})}
\end{equation*}
In the above, $\sigma_1 \succ \sigma_2$ indicates the event that segment 1 is preferred to segment 2. For a given dataset $\mathcal{D}$ comprised of labeled queries $(\sigma_1, \sigma_2, y)$ where $y= \{0, 1\}$ corresponds to whether $\sigma_0$ or $\sigma_1$ preferred, the following objective is optimized to learn $\hat{r}_\psi$.
\begin{equation} \label{eq:loss}
    \mathcal{L}_\text{pref} = - \E_{(\sigma^0, \sigma^1, y) \sim \mathcal{D}} \left[ y(0) \log (P[\sigma_0 \succ \sigma_1 ]) + y(1)\log(1 - P[\sigma_0 \succ \sigma_1 ]) \right]
\end{equation}
In practice, this is just the standard binary cross-entropy objective where logits are determined by the sum of the learned reward function $\sigma$ over $k$ timesteps. While in practice preferences over segments are provided by humans, preferences can also be induced by an oracle reward function $r(s_t, a_t)$. In simulated experiments it is common practice to generate labels $y$ via the comparison $\sum_t r(s^0_t, a^0_t) \overset{?}> \sum_t r(s^1_t, a^1_t)$ from an oracle reward function $r$.


